CHAMP: Efficient Annotation and Consolidation of Cluster Hierarchies

Various NLP tasks require a complex hierarchical structure over nodes, where each node is a cluster of items. Examples include generating entailment graphs, hierarchical cross-document coreference resolution, annotating event and subevent relations, etc. To enable efficient annotation of such hierarchical structures, we release CHAMP, an open source tool allowing to incrementally construct both clusters and hierarchy simultaneously over any type of texts. This incremental approach significantly reduces annotation time compared to the common pairwise annotation approach and also guarantees maintaining transitivity at the cluster and hierarchy levels. Furthermore, CHAMP includes a consolidation mode, where an adjudicator can easily compare multiple cluster hierarchy annotations and resolve disagreements.

==> sections/03_treecorefi.tex <==
\section{\tool{}}

% \ariec{Ido: change positioning -- we extend corefi to support the annotation of hierarchy of clusters + consolidation of text spans (not adding features)}





We enhance the original \textsc{CoRefi} annotation tool with two main features. First, we develop the ability to annotate a hierarchy of clusters~(§\ref{subsec:hierarchy}). Second, we develop an \textit{adjudication} mode that allows to effectively compare multiple annotations and build a consolidated hierarchy of clusters~(§\ref{subsec:adjudication}). This mode can be used by an adjudicator, which is usually a more reliable annotator, or by the original annotators during discussions to resolve conflicts. While \textsc{CoRefi} was initially introduced for annotating coreference clusters of mention spans in multiple texts, we extend this tool to encompass the annotation of any type of spans, including full statements. 

% We enhance the original \textsc{CoRefi} with two main features. We first develop the ability to \emph{manually} compare and consolidate the clustering annotation from multiple annotators~(§\ref{subsec:consolidation}). Second, we develop the ability to annotate and consolidate hierarchy of clusters in order to support the such annotation tasks~(§\ref{subsec:hierarchy}). Although \textsc{CoRefi} was initially introduced for annotating coreference clusters of mention spans in multiple texts, we extend this tool to encompass the annotation any type of spans, including full statements. 



\subsection{Cluster Hierarchy Annotation}
\label{subsec:hierarchy}

In this section, we describe how we extend \textsc{CoRefi} to allow the annotation of a hierarchy of clusters.

% \ariec{describe the annotation flow that we see in Figure 1}

A naive approach for supporting the annotation of such a structure would involve two separate steps: (1) clustering and (2) hierarchy construction over the fixed annotated clusters. However, this method lacks the flexibility for annotators to modify the clustering annotation while simultaneously working on the hierarchy, whereas typically many annotation decisions fall at the intersection of clustering and hierarchy~\citep{cattan2021scico}. Moreover, employing two separate annotation steps would burden annotators with the additional challenge of remembering the context of each cluster during hierarchy annotation. 
% Finally, this decoupling of clustering and hierarchy annotation would further complicate the consolidation process.

Therefore, we propose an \textit{incremental} approach for annotating both the clustering and the cluster hierarchy together as a single annotation task. At initialization, the first span is automatically assigned to the first cluster (in the cluster bank) and to a corresponding node in the hierarchy (see Figure~\ref{fig:hierarchy} at the bottom). Then, for each subsequent span $s$, the annotator first decides its cluster assignment, by choosing whether to assign $s$ to an existing or a new cluster. In the latter case, a new node is automatically created in the hierarchy under the root and the annotator can drag it to its right position in the current hierarchy. \ariec{explain the example in Figure 1}


\begin{figure*}[t]
     \centering
     \includegraphics[width=0.9\textwidth, frame]{images/hierarchy.png}
     \caption{User interface for annotating both clustering and hierarchical relations between clusters. The current statement to assign is underlined in purple: ``It's also very slow''. The annotator can decide whether to add it to an existing cluster (in which case it will concatenated in the corresponding node in the hierarchy and separated by ``;''), or to open a new cluster, (in which case a new node will be automatically added to the hierarchy under the root).}
     \label{fig:hierarchy}
\end{figure*}


Importantly, when the annotator re-assigns a previously assigned span to another cluster (as allowed in \textsc{CoRefi}), nodes and relations in the hierarchy will be automatically updated. Keeping in sync cluster assignments and hierarchy is not trivial because different clustering modifications will have different effect on the resulting hierarchy. For example, if the annotator re-assigns a span $s$ from a singleton cluster $C_i$ to a cluster $C_j$, the children of $C_i$ also need to be moved under $C_j$. On the other hand, if $s$ was moved from a non-singleton cluster $C_i$ to a cluster $C_j$, $C_i$'s children should likely stay under $C_i$. 

% Algorithm~\ref{algo:update_hierarchy} illustrates the process of the hierarchy update for each possible case of clustering re-assignment. 


% \input{sections/algo}



\subsection{Consolidation}
\label{subsec:adjudication}

% - what we do? 
% - why it's challenging? 
% - how we address it? 

In order to facilitate the manual adjudication of multiple hierarchy annotations, we develop a consolidation mode in \tool{} that aims to easily identify and highlight disagreements between multiple annotators. 

Comparing multiple annotations of a hierarchy of clusters can be challenging due to variations in annotators' clustering assignments, leading to different sets of nodes in the hierarchies. To illustrate this issue, consider a scenario where annotator A1 annotates the spans $(a, b, d) \xrightarrow{} (c, e)$, while A2 annotates $(a, b, z) \xrightarrow{} c$ and $(d, y) \xrightarrow{} e$, where the letters are mentions, parentheses denote clusters and arrows indicate hierarchical relations. The two hierarchies have similarities (e.g. both cluster $a$ and $b$ together and have $e$ a child of $d$) but differ in many other ways, and determining how to compare and adjudicate between such differing hierarchies is non-trivial. 

To tackle this problem, we suggest decoupling the consolidation into two consecutive steps: (1) clustering and (2) hierarchy. 

\begin{figure*}[t]
     \centering
     \includegraphics[width=0.9\textwidth, frame]{images/conscoref.png}
     \caption{Clustering consolidation. The thumb-down at the bottom left of the screen indicates a clustering disagreement between the annotators for the span \example{The directions also leave a lot to be desired}. Annotator A1 assigned it to \example{The device itself is so difficult to use} while annotator A2 created a new cluster, as indicated in purple.}
     \label{fig:cons1}
\end{figure*}

In the first step, the adjudicator is shown the spans in a sequential manner and can see, for each span, the cluster assignment of each of the original annotations. To determine the original clustering decisions of all annotators, we extend the reviewing mode in \textsc{CoRefi} (§\ref{subsec:bg_cons}) to simultaneously find the set of candidate clusters according to each original annotation. These candidates are presented to the adjudicator, displayed in purple at the bottom of the screen, as illustrated in Figure~\ref{fig:cons1}.





% apply the original token mapping algorithm of the \textsc{CoRefi}'s reviewing mode~(§\ref{sec:bg}) to all input annotations. 




% Figure~\ref{fig:cons1}\ariec{must change the figure} illustrates this process, with annotation disagreements clearly marked with a red thumb-down icon. 

In fact, resolving a clustering disagreement means that the adjudicator re-assigns a span to another cluster (or to a new cluster) for at least one of the annotators. Accordingly, we can apply the hierarchy update algorithm (Algorithm~\ref{algo:update_hierarchy}) in order to modify the nodes and hierarchical relations of the hierarchy nodes. Considering the example in Figure~\ref{fig:cons1} with a clustering disagreement for the span \example{The directions also leave a lot to be desired ($s_1$)}: annotator A1 grouped it together with \example{The device itself is so difficult to use ($s_2$)} whereas annotator A2 left it as a standalone node in the hierarchy (indicated by the + button in purple). Now, if the adjudicator decides to follow A1's decision, A2's original hierarchy will be automatically modified to include a grouped node \{\emph{The device itself is so difficult to use, The directions also leave a lot to be desired}\} (instead of two separated nodes) whose children will be the concatenation of the initial children of $s_1$ and $s_2$ (lines 2-3 in Algorithm~\ref{algo:update_hierarchy}). On the other hand, if the adjudicator decides to follow A2's decision, a new node \example{The directions also leave a lot to be desired} will be added in A1's hierarchy~(line 10 in Algorithm~\ref{algo:update_hierarchy}). In this case, the children of the initial grouped node will stay under \example{The device itself is so difficult to use}. This automatic process ensures that the modified hierarchies will include the exact same nodes at end of the clustering consolidation step.



% In order to facilitate the adjudication of multiple annotations, we introduce a new \textit{consolidation} mode in \tool{} that identifies and highlights disagreements between annotators. Similarly to the reviewing mode~(§\ref{sec:bg}), the adjudicator in the consolidation mode is shown the spans in a sequential manner and can see for each span, the cluster assignment of each of the original annotations. Figure~\ref{fig:cons1}\ariec{must change the figure} illustrates this process, with annotation disagreements clearly marked with a red thumb-down icon. 





% To achieve this, the consolidation mode takes as input multiple clustering assignments that were previously annotated individually, with no restriction on the number of annotations. To determine the original clustering decisions of all annotators for each span, we simultaneously apply the original token mapping algorithm to all input annotations. The resulting decisions are then presented to the adjudicator as candidates for the consolidation process. 




% - similar to the review, after we collect the individual annotation, we combine them and create a configuration file for consolidation


In the second step, as the set of nodes $\mathcal{V}$ in the hierarchies are identical, a disagreement arises when a node $v \in \mathcal{V}$ has a different direct parent in each hierarchy. To efficiently identify such discrepancies, the adjudicator can click on the ``Go To Next Disagreement'' button, which highlights the node $v$ in blue along with its direct parent in violet on all input hierarchies. As shown in Figure~\ref{fig:hierarchy_cons}, for instance, the node \example{Keyboard lacks expected keys for functionality} was placed under \example{Our computer never worked right from the start} by A1, and under \example{The device itself is so difficult to use} by A2. The adjudicator then assesses the correct hierarchical relation, updates the other hierarchies accordingly and moves on to the next disagreement. Once all hierarchical disagreements have been resolved, the structure of the initial hierarchies will be identical and the adjudicator can confidently submit their consolidated hierarchy.




\begin{figure*}[t]
     \centering
     \includegraphics[width=0.9\textwidth, frame]{images/hierarchy_cons.png}
     \caption{Annotation interface for the 2nd step of hierarchy consolidation}
     \label{fig:hierarchy_cons}
\end{figure*}

==> sections/algo.tex <==
\definecolor{mygray}{gray}{0.2}
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{mygray}{#1}}
\SetCommentSty{mycommfont}


\begin{algorithm}
\SetAlgoLined
\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead


\KwIn{$source | C_{source} \in$ \{\text{singleton, non-singleton}\}, \\ $dest | C_{dest} \in$ \{\text{singleton, non-singleton, new-cluster}\}}
% \KwOut{$A$: Action} 
\BlankLine

 \If{isSingleton($C_{source}$)}{
      moveChildren($children(C_{source})$, $C_{dest}$)\;
      moveSpanToNode($source$, $C_{dest}$)\;
}\Else(\tcp*[h]{non-singleton}) { 
    \If{$C_{dest} \in$ \{singleton, non-singleton\}} {
        moveSpanToNode($source$, $C_{dest}$)\;
    }
    \Else(\tcp*[h]{new cluster}) { 
        createNode($source$, $par(C_{source})$)
    }
} 
\caption{Automatic hierarchy update after the span $source$ was re-assigned to the cluster $C_{dest}$. }
\label{algo:update_hierarchy}
\end{algorithm}
